MadRadar: A Black-Box Physical Layer Attack Framework on mmWave Automotive FMCW Radars

Frequency modulated continuous wave (FMCW) millimeter-wave (mmWave) radars play a critical role in many of the advanced driver assistance systems (ADAS) featured on today's vehicles. While previous works have demonstrated (only) successful false-positive spoofing attacks against these sensors, all but one assumed that an attacker had the runtime knowledge of the victim radar's configuration. In this work, we introduce MadRadar, a general black-box radar attack framework for automotive mmWave FMCW radars capable of estimating the victim radar's configuration in real-time, and then executing an attack based on the estimates. We evaluate the impact of such attacks maliciously manipulating a victim radar's point cloud, and show the novel ability to effectively `add' (i.e., false positive attacks), `remove' (i.e., false negative attacks), or `move' (i.e., translation attacks) object detections from a victim vehicle's scene. Finally, we experimentally demonstrate the feasibility of our attacks on real-world case studies performed using a real-time physical prototype on a software-defined radio platform.

==> 07b_mmWave_Case_Studies.tex <==
\vspace{-8pt}
\section{Off-the-Shelf mmWave Radar Case Studies}
\label{07a_mmWave_Case_studies}
\vspace{-8pt}

% In section \ref{07_Experimental_Results}, we validated the feasibility and performance of our black box attack architecture using a software-defined radio platform. However, we were unable to perform experiments at mm-Wave frequencies due to hardware limitations. As such, 
Finally, we performed additional case studies using commercially available mm-Wave radar development boards to demonstrate %what our attacks would look like 
the effectiveness of the developed black-box attacks against state-of-the-art automotive radars. Due to the hardware limitations of the  mm-Wave development boards we used~\cite{texas_instruments_iwr1443_2018}, we were unable to implement the real-time estimation component of our black-box attack.  %Given these limitations, 
Instead, we had to utilize an external clock to synchronize the victim and attacker radars, and we assumed that the attacker had already 
estimated %offline 
the victim's radar parameters with the estimation errors obtained in our analysis in the previous sections.  % when performing these case studies. 
Additionally, our ability to specify an exact spoofing velocity for the attack was limited by the phase shifters on the development boards. Still, combined with our previous simulations and experiments, these case studies show that our attacks could be implemented against actual automotive~radars.


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.52\columnwidth]{figures/07_mmWave_experimental_setup.png}
    \vspace{-8pt}
    \caption{Experimental Setup for mmWave Case Studies.}
    \label{fig_07a_mmWave_experimental setup}
    \vspace{-8pt}
\end{figure}

\vspace{-12pt}
\paragraph{Experimental Setup.}
We used the TI IWR1443 radar development boards both as our victim radar and attacker since it is a good representation of the hardware commonly found in automotive radars~\cite{texas_instruments_iwr1443_2018}. The victim and attacker were synchronized using a Tektronix AFG3052C dual-channel function generator \cite{tektronix_afg30000c_nodate}. Additionally, we utilized the TI-DCA1000 data capture card~\cite{texas_instruments_users_2019} on the victim to capture victim frames. 

The victim radar was programmed using TI's mmWave Studio. % from Texas Instruments. 
Once the victim's parameters were set, we utilized the TI's Demo Visualizer web application to load %a nearly identical (simulating parameter estimation) 
the estimated configuration to the TI-IWR1443 radar representing the attacker. Both the attacker and victim were set to "Hardware Trigger" mode to meet the precise timing requirements for our attacks. Finally, the distance of the attack was set by adjusting the frame start trigger delay in mmWave Studio to the timing delay required for a specific spoofing distance. The entire setup was placed on a mobile cart so that we could perform field tests with actual vehicles (see Fig. \ref{fig_07a_mmWave_experimental setup} setup). % shows the experimental setup that was used for our case studies.
% \todo{check the whole subsection} \todo{MP - check: section looks good, just want to make sure that this is demonstrating the attacks, and not demonstrating anything to do with parameter estimation}


\begin{figure}[!t]
     \centering
     \begin{subfigure}[b]{0.48\columnwidth}
         \centering
         \includegraphics[width=0.86\columnwidth]{figures/07_mmWave_spoof.png}
         \caption{FP Spoofing Attack}
         \label{fig_07a_mmWave_spoof}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\columnwidth}
         \centering
         \includegraphics[width=0.86\columnwidth]{figures/07_mmWave_noisy.png}
         \caption{FN Noisy Velocity Attack}
         \label{fig_07a_mmWave_noisy}
     \end{subfigure}
     \vspace{-8pt}
        \caption{Range Doppler Plots for mmWave Case Studies.}
        \label{fig_07a_mmWave_Range_Dopplers}
\end{figure}


\vspace{-12pt}
\paragraph{Results.}
Fig. \ref{fig_07a_mmWave_Range_Dopplers} shows the Range Doppler plots %that we 
recorded for two of our case studies. As shown in Fig. \ref{fig_07a_mmWave_spoof}, the victim observed a real target (a bus in this case) at $10 m$ traveling $10 m/s$ towards the radar. However, the attack also added an additional spoofed object at $10 m$ traveling with a relative velocity of $10 m/s$ away from the radar. As previously discussed, the spoofed object is still smeared in the range domain due to the attack's chirp slope being slightly different than the victim's chirp~slope. 

Fig. \ref{fig_07a_mmWave_noisy} features the Range Doppler plot for a noisy velocity FN attack. %As seen here, we were 
The attack was able to add noise across the velocity bins at $3 m$ of range, which would prevent object detection. While we were unable to concentrate this attack at a specific velocity due to hardware constraints, the range doppler plot still shows that the attack is feasible at mm-Wave frequencies, %. While we were limited by the hardware capabilities in our implementation, these results indicate that such an attack 
and that it could be implemented %if someone had 
with access to the required hardware. For example, a high-end RFSOC (RF System on a Chip) board combined with a custom RF frequency conversion chain, could be used to implement the full-scale black-box attack on mm-Wave radars, but % even though 
such an implementation would cost tens of thousands of dollars.

